Geometry of Rounding: Near Optimal Bounds and a New Neighborhood Sperner's Lemma

A partition $\mathcal{P}$ of $\mathbb{R}^d$ is called a $(k,\varepsilon)$-secluded partition if, for every $\vec{p} \in \mathbb{R}^d$, the ball $\overline{B}_{\infty}(\varepsilon, \vec{p})$ intersects at most $k$ members of $\mathcal{P}$. A goal in designing such secluded partitions is to minimize $k$ while making $\varepsilon$ as large as possible. This partition problem has connections to a diverse range of topics, including deterministic rounding schemes, pseudodeterminism, replicability, as well as Sperner/KKM-type results. In this work, we establish near-optimal relationships between $k$ and $\varepsilon$. We show that, for any bounded measure partitions and for any $d\geq 1$, it must be that $k\geq(1+2\varepsilon)^d$. Thus, when $k=k(d)$ is restricted to ${\rm poly}(d)$, it follows that $\varepsilon=\varepsilon(d)\in O\left(\frac{\ln d}{d}\right)$. This bound is tight up to log factors, as it is known that there exist secluded partitions with $k(d)=d+1$ and $\varepsilon(d)=\frac{1}{2d}$. We also provide new constructions of secluded partitions that work for a broad spectrum of $k(d)$ and $\varepsilon(d)$ parameters. Specifically, we prove that, for any $f:\mathbb{N}\rightarrow\mathbb{N}$, there is a secluded partition with $k(d)=(f(d)+1)^{\lceil\frac{d}{f(d)}\rceil}$ and $\varepsilon(d)=\frac{1}{2f(d)}$. These new partitions are optimal up to $O(\log d)$ factors for various choices of $k(d)$ and $\varepsilon(d)$. Based on the lower bound result, we establish a new neighborhood version of Sperner's lemma over hypercubes, which is of independent interest. In addition, we prove a no-free-lunch theorem about the limitations of rounding schemes in the context of pseudodeterministic/replicable algorithms.

==> _watermark.tex <==
\usepackage{draftwatermark}
\SetWatermarkText{DRAFT}
%\SetWatermarkText{DRAFT:\\DO NOT\\DISTRUBUTE}
\SetWatermarkLightness{0.95}
\SetWatermarkScale{7}
% \SetWatermarkScale{3.5}

==> images/sperner_kkm_lebesgue/OLD/figure_code.tex <==
% This looks more complicated than normal in order to display the figure numbers with priority for moving down the columns instead of across the rows. 
% https://tex.stackexchange.com/questions/235690/i-want-to-change-the-order-of-numbering-for-captions-in-subfigure
% https://tex.stackexchange.com/questions/31823/how-to-reference-subfigure-in-caption
\begin{figure}[p]
\sbox0{%
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/0_non-spanning_coloring.png}
        \subcaption{Initial coloring $\chi_0$}
        \label{subfig:0_non-spanning_coloring}
    \end{subfigure}
}
\sbox1{%
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/1_sperner_kkm_coloring.png}
        \subcaption{Modified coloring $\chi$}
        \label{subfig:1_sperner_kkm_coloring}
    \end{subfigure}
}
\sbox2{%
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/2_extended_sperner_kkm_coloring.png}
        \subcaption{Extended coloring $\gamma$}
        \label{subfig:2_extended_sperner_kkm_coloring}
    \end{subfigure}
}
\sbox3{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/5_isolated_purple.png}
        \subcaption{Color $\langle -1,-1 \rangle$ (purple)}
        \label{subfig:5_isolated_purple}
    \end{subfigure}
}
\sbox4{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/6_minkowski_sum_purple_new.png}
        \subcaption{Ball added to color}
        \label{subfig:6_minkowski_sum_purple}
    \end{subfigure}
}
\sbox5{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/3_isolated_red.png}
        \subcaption{Color $\langle -1,1 \rangle$ (red)}
        \label{subfig:3_isolated_red}
    \end{subfigure}
}
\sbox6{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/4_minkowski_sum_red_new.png}
        \subcaption{Ball added to color}
        \label{subfig:4_minkowski_sum_red}
    \end{subfigure}
}
\sbox7{%
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/blank_square.png}
    \end{subfigure}
}
\sbox8{%
    \begin{subfigure}{.15\textwidth}
        \includegraphics[width=\textwidth]{images/blank_square.png}
    \end{subfigure}
}

\centering
% \usebox0 \hfill \usebox7 \hfill \usebox7
% \usebox1 \hfill \usebox3 \hfill \usebox5
% \usebox2 \hfill \usebox4 \hfill \usebox6

% \usebox0 \hfill \usebox7 \hfill \usebox7
% \usebox1 \hfill \usebox7 \hfill \usebox7
% \usebox2 \hfill \usebox3 \hfill \usebox5
% \usebox7 \hfill \usebox4 \hfill \usebox6

% \usebox0 \hfill \usebox1 \hfill \usebox2
% \usebox2 \hfill \usebox3 \hfill \usebox5
% \usebox2 \hfill \usebox4 \hfill \usebox6

\usebox0 \hfill \usebox1 \hfill \usebox2
\usebox8 \hfill \usebox3 \hfill \usebox4 \hfill \usebox8
\usebox8 \hfill \usebox5 \hfill \usebox6 \hfill \usebox8

\caption{
\subref{subfig:1_sperner_kkm_coloring} shows a Sperner/KKM coloring of the unit cube $[-\frac12,\frac12]^2$. All points on an edge are colored with one of the two colors matching the vertices defining that edge. 
%
\subref{subfig:2_extended_sperner_kkm_coloring} shows the extension of that coloring to $[-\frac12-\epsilon,\frac12+\epsilon]^2$. The extension is obtained by mapping each point $\vec{x}$ to the point $\vec{x}'$ in which each coordinate value is restricted to be within $[-\frac12,\frac12]$, and then $\vec{x}$ is given whatever color $\vec{x}'$ had.
%
\subref{subfig:3_isolated_red} shows the set corresponding to the color $\vec{c}=\langle -1,1 \rangle$ (shown in red) and shows the open ball $B_{\vec{c}}$ which is Minkowski summed with this set. The color is the top left color, so the representative point of $B_{\vec{c}}$ (i.e. the origin) is also at the top left. Note that the set is $\epsilon$ far away from the right edge and the bottom edge.
%
\subref{subfig:4_minkowski_sum_red} shows the Minkowski sum of this color set and the ball. Note that it is a subset of $[-\frac12-\epsilon,\frac12+\epsilon]^2$. Also, it has substantially more area---by a factor of at least $(1+\frac{\epsilon}{1+\epsilon})^2\geq(1+\frac32\epsilon)^2$.
%
\subref{subfig:5_isolated_purple} is analogous to \subref{subfig:3_isolated_red} but showing the color $\vec{c}=\langle -1,-1 \rangle$ (shown in purple). Note the open ball $B_{\vec{c}}$ has a different representative point.
%
\subref{subfig:6_minkowski_sum_purple} is analogous to \subref{subfig:4_minkowski_sum_red}.
}

\label{fig:sperner-kkm-coloring}

\end{figure}

==> partition_classes.tex <==
\section{Some Classes of Partitions}

\todo[inline]{Discuss the recursive tower structure view of the reclusive partitions}

In exploring upper and lower bounds on the reclusive partitions specifically, we have found frequently that we make use of one of three structural properties of those partitions.
In this section we give precise definitions to capture these three different properties so that results we would otherwise prove only of the reclusive can instead be just as easily proved in a generalized setting. Toward this goal, we will define six types of partitions to capture these structures and then explore/prove the hierarchy of these partitions shown in \Autoref{fig:partition-type-hierarchy}. Recall that the three structures of the reclusive partitions that we have utilized are (1) the algebraic structure provided by the defining matrix and the group theoretic lattice structure it induces, (2) the layered structure of the partitions given by the view of building the partition one dimension at a time and building the next dimension by extruding the prior partition and then shifting it by different amounts in infinitely many layers to partition the next dimension, and (3) the tower structure that arises from a different view of iteratively constructing the partition one dimension at a time, by building a new dimension by turning every cube in the prior partition into an infinite tower of cubes moving up and down in the new coordinate. The big idea of the six definitions will be as follows:

\begin{description}
\item[Tower Unit Cube Partition:] A unit cube partitions where there is some coordinate $i_0$ such that the partition consists of infinite towers of cubes along coordinate $i_0$. In other words, for every cube $X$ in the partition, for every $n\in\Z$, there is also a cube centered at $\centr(X)+n\cdot\stdbasis{i_0}$, so the partition consists entirely of these infinite towers of cubes. Furthermore, viewing the union of cubes in each tower as the product of $\R$ and a cube of one dimension lower, these partitions naturally give rise to a unit cube partition of one dimension lower.

% \item[Recursive Tower Unit Cube Partition: ] A tower unit cube partition such that after applying a natural projection operation (reducing each tower to a single cube in one lower dimension) gives another tower unit cube partition, and this can be done iteratively to get a tower unit cube partition for each dimension $d,d-1,d-2,\ldots,3,2,1$.
\item[Recursive Tower Unit Cube Partition:] This is inductively defined so that any unit cube partition of $\R^1$ is a recursive tower unit cube partition. For higher dimensions, a recursive tower unit cube partition is a tower unit cube partition such that the natural partition of one dimension lower that it gives rise to is also a recursive tower unit cube partition. This type of unit cube partition is useful for inductive proofs since you can ``peel away`` one dimension and still have all of the same structural properties remaining.

\item[Layer Unit Cube Partition:] A unit cube partition where there is some coordinate $i_0$ such that (morally) all cubes have integral $i_0$th coordinate. Thus, the partition consists of one layer of cubes for each integer $n\in\Z$ (the $n$th layer consisting of all cubes with $i_0$th coordinate equal to $n$). Furthermore, each layer $n$ naturally induces a unit cube partition of one dimension smaller by looking at how the cubes in layer $n$ intersect the hyperplane of all points in $\R^d$ with $i_0$th coordinate $n$.

\item[Recursive Layer Unit Cube Partition:] This is inductively defined so that any unit cube partition of $\R^1$ is a recursive tower unit cube partition. For higher dimensions, a recursive layer unit cube partition is a layer unit cube partition such that for each layer, the natural partition of one dimension lower that it gives rise to is also a recursive layer unit cube partition. Again, this type of unit cube partition is useful for inductive proofs since the partition consists of layers of partitions which also carry the same structure.

\item[Lattice Unit Cube Partition:] A unit cube partition where the positions (i.e. centers) of each cube form a lattice (a lattice has two equivalent definitions, one is a group theory structure and one is a linear algebraic structure).

\item[Single Set Lattice Partition:] This is a generalization of lattice unit cube partitions in which the members do not have to be unit cubes. Instead there is some set $S$, and each members of the partition is some shift of $S$ such that all positions of $S$ in the partition form a lattice. 
\end{description}

\todo[inline]{defn}
\begin{definition}[Unit Cube Partition]
Let $d\in\N$. A {\em unit cube partition} of $\R^d$ is a partition $\P$ of $\R^d$ such that for each $X\in\P$, there is some $\vec{\alpha}\in\R^d$ such that $X=\vec{\alpha}+[0,1)^d$.
\end{definition}

\todo[inline]{Induced hyperplane partition}
When the dimension $d$ is understood, we will use the notation $\hp{i}{\alpha}$ to denote the hyperplane in $\R^d$ given by the set of points $\set{\vec{x}\in\R^d\colon x_i=\alpha}$, and for any partition $\P$ of $\R^d$, we let $\P_{\hp{i}{\alpha}}$ denote the partition of the hyperplane induced by $\P$.

\begin{definition}[Tower Unit Cube Partition]
Let $d\in\N$. A {\em tower unit cube partition} of $\R^d$ is a unit cube partition $\P$ of $\R^d$ such that there exists $i_0\in[d]$ (not necessarily unique) such that for any cube $X\in\P$, the set $X+\stdbasis{i_0}$ is also a member of $\P$. Such $i_0$ is called a {\em tower coordinate}.
\end{definition}

\begin{remark}
The condition that $X+\stdbasis{i_0}$ is a member of $\P$ could have also been stated as ``there exists $Y\in\P$ such that $\centr(Y)=\centr(X)+\stdbasis{i_0}$.
\end{remark}

It trivially follows from the definition above that for any $X\in\P$, it holds for every $n\in\N$ that $X+n\cdot\stdbasis{i_0}$ is a member of $\P$ (just apply the definition $n$ times). However, in the motivation we said we wanted this to hold for all $n\in\Z$. By the same reasoning, it is sufficient that $X-\cdot\stdbasis{i_0}$ is a member of $\P$. We show in the next result that this property follows from the definition above.

\todo[inline]{Add center-locality-lemma}
\begin{lemma}[Negative Direction Tower]
Let $d\in\N$, $\P$ a tower unit cube partition of $\R^d$, and $i_0\in[d]$ a tower coordinate of $\P$. Then for any cube $X\in\P$, $X-\stdbasis{i_0}$ is also a member of $\P$.
\end{lemma}
\begin{proof}
Let $X\in\P$ be arbitrary. Consider the regions
\begin{align*}
    R_Y &= \centr(X)-\stdbasis{i_0}+[-\frac12,\frac12)\\
    R_X &= \centr(X)+[-\frac12,\frac12) = R_Y+\stdbasis{i_0}
\end{align*} 
(so actually $R_X=X$, but conceptually we will think of $R_X$ as a region in space rather than as a member of $\P$). By \Autoref{center-locality-lemma}, there is a (unique) cube $Y\in\P$ such that $\centr(Y)\in R_Y$. Let $X'=Y+\stdbasis{i_0}$. Since $\P$ is a tower unit cube partition, $X'\in\P$. Now observe that since $\centr(Y)\in R_Y$,
\[
\centr(X') = \centr(Y+\stdbasis{i_0}) = \centr(Y)+\stdbasis{i_0} \in R_Y+\stdbasis{i_0} = R_X
\]
showing that $\centr(X')\in R_X$. Also (trivially), $\centr(X)\in R_X$. By \Autoref{center-locality-lemma}, there is a unique member of $\P$ with its center in $R_X$, so $X=X'=Y+\stdbasis{i_0}$. Thus, $X-\stdbasis{i_0}=Y$ and by construction $Y\in\P$.
\end{proof}

Together, the next two results show that we can in fact do what we expect to be able to do, and project all cubes in a tower unit cube partition along a tower coordinate to obtain a unit cube partition of one dimension lower.

\begin{lemma}[Projections of Tower Cubes 1]\label{projections-of-tower-cubes-1}
Let $d\in\N$, $\P$ a tower unit cube partition of $\R^d$, and $i_0\in[d]$ a tower coordinate of $\P$. Then for any cubes $X,Y\in\P$, either $\tau_{i_0}(X)=\tau_{i_0}(Y)$ or $\tau_{i_0}(X)\cap\tau_{i_0}(Y)=\emptyset$.
\end{lemma}
\begin{proof}
Let $X,Y\in\P$ be arbitrary. Let $\mathcal{T}=\set{X+n\cdot\stdbasis{i_0}:n\in\Z}\subseteq\P$ which represents all cubes in the tower with $X$. If $Y\in\mathcal{T}$, then there is some $n_Y\in\Z$ such that $Y=X+n_Y\cdot\stdbasis{i_0}$ so
\begin{align*}
    \tau_{i_0}(X) &= \set{\tau_{i_0}(\vec{x}): \vec{x}\in X} \tag{Def'n of projection of set} \\
    &= \set{\tau_{i_0}(\vec{x}+n_Y\cdot\stdbasis{i_0}): \vec{x}\in X} \tag{$\tau_{i+0}$ ignores the $i_0$th coordinate} \\
    &= \set{\tau_{i_0}(\vec{y}): \vec{y}\in Y} \tag{$Y=X+n_Y\cdot\stdbasis{i_0}$} \\
    &= \tau_{i_0}(Y) \tag{Def'n of projection of set}
\end{align*}

Otherwise, $Y\not\in\mathcal{T}$. Let $T=\bigcup_{Z\in T}Z$ noting that
\[
T = \prod_{i=1}^d
\begin{cases}
    \centr_i(X)+[-\frac12,\frac12) & i\not=i_0 \\
    \R                             & i=i_0
\end{cases}
\]
Since $\P$ is a partition and $Y\not\in\mathcal{T}$, we have $Y\cap T\not=\emptyset$. Thus, there is some\footnote{One might note that if $d=1$, then $[d]\setminus\set{i_0}$ is empty so it must be that $Y\in\mathcal{T}$ and $\tau_{i_0}(X)=\tau_{i_0}(Y)$.}  $i_1\in[d]\setminus\set{i_0}$ such that $\abs{\centr_{i_1}(X)-\centr_{i_1}(Y)}\geq1$, and thus $\centr(\tau_{i_0}(X))=\tau_{i_0}(\centr(X))$ and $\centr(\tau_{i_0}(Y))=\tau_{i_0}(\centr(Y))$ also differ by at least $1$ in the coordinate corresponding to $i_1$, so $\tau_{i_0}(X)\cap\tau_{i_0}(Y)=\emptyset$.
\end{proof}


\begin{lemma}[Projections of Tower Cubes 2]
Let $d\in\N$, $\P$ a tower unit cube partition of $\R^d$, and $i_0\in[d]$ a tower coordinate of $\P$. Then the set $\P'=\set{\tau_{i_0}(X)\colon X\in\P}$ is a unit cube partition of $\R^{d-1}$.
\end{lemma}
\begin{proof}
First, we show $\P'$ covers $\R^{d-1}$. Let $\vec{x}'\in\R^{d-1}$ be arbitrary, and take $\vec{x}$ to be any point in $\tau_{i_0}^{-1}(\vec{x}')$ (i.e., $\vec{x}$ is some point of $\R^d$ that is mapped to $\vec{x}'$ by $\tau_{i_0}$). Then because $\P$ is a partition of $\R^d$, there exists some (unique) $X\in\P$ with $\vec{x}\in X$. Let $X'=\tau_{i_0}(X)\in\P'$. Thus
\[
\vec{x}' = \tau_{i_0}(\vec{x}) \in \tau_{i_0}(\vec{X}) = X' \in \P'
\]
showing that $\vec{x}'$ belongs to some member of $\P'$.

Second, we show that no two members of $\P'$ intersect. Let $X',Y'\in\P'$ be distinct. By definition of $\P'$, let $X\in\P$ be some member such that $X'=\tau_{i_0}(X)$, and let $Y\in\P$ be some member such that $Y'=\tau_{i_0}(Y)$. Since $\tau_{i_0}(X)=X'\not=Y'=\tau_{i_0}(Y)$, we have by \Autoref{projections-of-tower-cubes-1} that $\tau_{i_0}(X)\cap\tau_{i_0}(Y)=\emptyset$, so $X'\cap Y'=\emptyset$.
\end{proof}

Now we give the definition of a {\em recursive} tower unit cube partition which remands the tower unit cube partition structure through all induced partitions of lower dimensions.

\begin{definition}[Recursive Tower Unit Cube Partition]
A {\em recursive tower unit cube partition} of $\R^1$ is any tower unit cube partition of $\R^1$ (and therefore any unit cube partition of $\R^1$). For $d\in\N$, $d>1$, a {\em recursive tower unit cube partition} of $\R^d$ is a tower unit cube partition $\P$ of $\R^d$ such that there is at least one tower coordinate $i_0\in[d]$ for which the unit cube partition $\P'=\set{\tau_{i_0}(X)\colon X\in\P}$ of $\R^{d-1}$ is in fact a recursive tower unit cube partition.
\end{definition}

\begin{definition}[Layer Unit Cube Partition]
Let $d\in\N$. A {\em layer unit cube partition} of $\R^d$ is a unit cube partition $\P$ of $\R^d$ such that there exists some $\alpha\in\R$ and some $i_0\in[d]$ such that for each $X\in\P$, $\centr_{i_0}(X)\in\alpha+\Z$. Such $i_0$ is called a {\em layer coordinate}.
\end{definition}

\begin{definition}[Recursive Layer Unit Cube Partition]
A {\em recursive layer unit cube partition} of $\R^1$ is any layer unit cube partition of $\R^1$ (and therefore any unit cube partition of $\R^1$). For $d\in\N$, $d>1$, a {\em recursive layer unit cube partition} of $\R^d$ is a layer unit cube partition $\P$ of $\R^d$ such that there is at least one layer coordinate $i_0\in[d]$ such that for all $\alpha\in\R$, the unit cube partition $\P_{\hp{i_0}{\alpha}}$ is in fact a recursive layer unit cube partition.
\end{definition}

\begin{remark}[Equivalent Definition of Recursive Layer Unit Cube Partition]
Probably a more natural, but equivalent, definition would have been to require that for $d\in\N$, $d>1$, a {\em recursive layer unit cube partition} of $\R^d$ is a layer unit cube partition $\P$ of $\R^d$ such that there is at least one layer coordinate $i_0\in[d]$ and associated $\alpha'\in\R$ (i.e. $\set{\centr_{i_0}(X)\colon X\in\P}=\alpha+\Z$) such that for each $n\in\Z$, the set $\P'=\set{\tau_{i_0}(X)\colon X\in\P\text{ and }\centr_{i_0}(X)=\alpha+n}$ is in fact a recursive layer unit cube partition.

This definition better captures the conceptual idea that the partition consists of layers and each layer is itself (after projecting out the appropriate coordinate) a recursive layer unit cube partition. We won't formally prove that these definitions are the same as we will always use the stated definition.
\end{remark}

\begin{definition}[Lattice Unit Cube Partition]
Let $d\in\N$. A {\em lattice unit cube partition} of $\R^d$ is a partition $\P$ of $\R^d$ such that the set $\set{\centr(X)\colon X\in\P}$ is a lattice.
\end{definition}

\begin{remark}
We could alter the definition above to allow that there is some $\vec{\alpha}\in\R^d$ such that $\vec{\alpha}+\set{\centr(X)\colon X\in\P}$ is a lattice. However, this doesn't allow for any interesting structure because it is just a shift of a lattice partition. However, in the definition of a recursive layer unit cube partition, it was absolutely necessary to include in the definition the allowance for a parameter $\alpha$, because otherwise a simple inductive proof would show that the only partition of $\R^d$ which would be considered recursively layered would be the standard grid partition.
\end{remark}

\begin{definition}[Single Set Lattice (Unit) Partition]
% Let $d\in\N$. A {\em unit cube partition} of $\R^d$ is a partition $\P$ of $\R^d$ such that for each $X\in\P$, there is some $\vec{\alpha}\in\R^d$ such that $X=\vec{\alpha}+[0,1)^d$.
\end{definition}

\todo[inline]{Formalize}
\begin{proposition}
A reclusive partition satisfies all 6 definitions above
\end{proposition}

We think of lattice unit cube partitions as very natural. In light of \todo[inline]{Reference result saying tilings and partitions are the same}, lattice unit cube partitions were one of the earliest unit cube partitions of interest, as they were the subject of Minkowski's conjecture from \todo[inline]{state year and fill in Minkowski's conjecture} which was proved in \todo[inline]{State name Hajos, year, and cite paper}

\begin{theorem}[Minkowski's Conjecture]\label{minkowskis-conjecture}
Let $d\in\N$, and $\mathcal{P}$ be a lattice unit cube partition of $\R^d$. Then there exists a pair of cubes whose closures intersect in a $(d-1)$-dimensional facet of each.
\end{theorem}

For this reason, we view lattice unit cube partitions as very natural objects of study. However, it is less clear that we should consider recursive tower unit cube partitions and recursive layer unit cube partitions as natural objects of study in their own right. Mostly they were defined to capture different aspects of the structure of the reclusive partitions defined in \todo[inline]{cite our first paper}. However, it turns out that not only did the reclusive partitions have both of these structures, but in fact every lattice unit cube partition is both a recursive tower unit cube partition and a recursive layer unit cube partition. Thus, if one is willing to consider lattice unit cube partitions a natural object of study, then they must concede that recursive tower unit cube partitions and recursive layer unit cube partitions are as well as they can both highlight specific structure in lattice unit cube partitions and serve as generalizations of lattice unit cube partitions\footnote{In a forthcoming paper we study partitions which surprisingly turn out to be recursive layer unit cube partitions which gives further evidence of the usefulness of this definition.}. We will first prove that every recursive tower unit cube partition is a recursive layer unit cube partition (\Autoref{recursive-tower-is-recursive-layer}) and then prove that every lattice unit cube partition is a recursive tower unit cube partition (\Autoref{lattice-is-recursive-tower}). We also provide an example demonstrating that the recursive structure is necessary in the first of these proofs---though recursive tower unit cube partitions must be recursive layer unit cube partitions, tower unit cube partitions need not be layer unit cube partitions (\Autoref{tower-not-layer}). We begin with a useful lemma.

\todo[inline]{Include implication diagram}

\begin{lemma}[Recursive Tower $\Longrightarrow$ Recursive Tower Hyperplanes]\label{recursive-tower-to-hyperplane}
Let $d\in\N$ and $\P$ a recursive tower unit cube partition of $\R^d$. Let $i_0\in[d]$ and $\alpha\in\R$ be arbitrary. Then either $d=1$ or $\P_{\hp{i_0}{\alpha}}$ is a recursive tower unit cube partition of $\R^{d-1}$.
\end{lemma}
\begin{proof}
We prove this by induction on $d$. If $d=1$, then we are trivially done, so we proceed assuming the inductive hypothesis.

If $i_0$ is a tower coordinate of $\P$, then by \todo[inline]{write and cite fact that in a tower unit cube partitions with tower coordinate $i_0$, the projection partition along $i_0$ is identical to any induced hyperplane partition for coordinate $i_0$.}, $\P_{\hp{i_0}{\alpha}}=\set{\tau_{i_0}(X)\colon X\in\P}$ which is a recursive tower unit cube partition by definition of $\P$ being a recursive tower unit cube partition.

Otherwise, $i_0$ is not a tower coordinate, so let $i_1$ be a tower coordinate for $\P$ which necessarily differs from $i_0$. Conceptually, the remainder of the proof shows that the projection along coordinate $i_1$ and the intersection of the coordinate $i_0$ hyperplane are operations that commute.

Let $\P'=\set{\tau_{i_1}(X)\colon X\in\P}$ which is a recursive tower unit cube partition by definition of $\P$ being a recursive tower unit cube partition. Since $\P'$ is a partition of $\R^{d-1}$, by inductive hypothesis, $\P'_{\hp{i_0}{\alpha}}$ is a recursive tower unit cube partition. Thus, we will be done with the proof if we show that
\[
\set{\tau_{i_1}(Y)\colon Y\in \P_{\hp{i_0}{\alpha}}} = \P'_{\hp{i_0}{\alpha}}
\]
as this shows by \todo[inline]{write and reference result that partition is a tower partition if and only if the projection is a partition} that $\P_{\hp{i_0}{\alpha}}$ (the partition we are interested in) is a tower unit cube partition with tower coordinate $i_1$ and that the set of $\tau_{i_1}$ projections is a recursive tower unit cube partition (since $\P'_{\hp{i_0}{\alpha}}$ is). Thus, we demonstrate this equality below:
\begin{align*}
    \set{\tau_{i_1}(Y)\colon Y\in\P_{\hp{i_0}{\alpha}}} &=     \Big\{\tau_{i_1}(Y)\colon Y\in\set{\tau_{i_0}(X)\colon X\in\P\text{ and }\alpha\in\pi_{i_0}(X)}\Big\} \tag{Def'n of $\P_{\hp{i_0}{\alpha}}$} \\
    %
    &= \Big\{\tau_{i_1}(\tau_{i_0}(X))\colon X\in\P\text{ and }\alpha\in\pi_{i_0}(X)\Big\} \tag{Set equality} \\
    %
    &= \Big\{\tau_{i_0}(\tau_{i_1}(X))\colon X\in\P\text{ and }\alpha\in\pi_{i_0}(X)\Big\} \tag{Projections commute} \\
    %
    &= \Big\{ \tau_{i_0}(Z)\colon Z\in\set{\tau_{i_1}(X)\colon X\in\P\text{ and }\alpha\in\pi_{i_0}(X)} \Big\} \tag{Set equality} \\
    %
    &= \Big\{ \tau_{i_0}(Z)\colon Z\in\set{\tau_{i_1}(X)\colon X\in\P\text{ and }\alpha\in\pi_{i_0}(\tau_{i_1}(X))} \Big\} \tag{Projection in $i_0$ unaffected by removal of $i_1$th coord since $i_0\not=i_1$} \\
    %
    &= \Big\{ \tau_{i_0}(Z)\colon Z\in\set{\tau_{i_1}(X)\colon X\in\P}\text{ and }\alpha\in\pi_{i_0}(Z) \Big\} \tag{Set equality} \\
    %
    &= \Big\{ \tau_{i_0}(Z)\colon Z\in\P'\text{ and }\alpha\in\pi_{i_0}(Z) \Big\} \tag{Def'n of $\P'$} \\
    %
    &= \P'_{\hp{i_0}{\alpha}} \tag{Equiv def'n of induced hyperplane partition}
\end{align*}
\end{proof}

\begin{proposition}[Recursive Tower $\Longrightarrow$ Recursive Layer]\label{recursive-tower-is-recursive-layer}
Let $d\in\N$ and $\P$ a recursive tower unit cube partition of $\R^d$. Then $\P$ is also a recursive layer unit cube partition of $\R^d$.
\end{proposition}
\begin{proof}
We prove this by induction on $d$. The base case of $d=1$ is trivial because every recursive tower unit cube partition of $\R^1$ is a unit cube partition of $\R^1$, and every unit cube partition of $\R^1$ is a recursive layer unit cube partition of $\R^1$ by definition.

For the inductive case, because $\P$ is a recursive tower unit cube partition, there exists some tower coordinate $i_0\in[d]$ so that $\P'=\set{\tau_{i_0}(X)\colon X\in\P}$ is a recursive tower unit cube partition of $\R^{d-1}$. By inductive hypothesis, this is a recursive layer unit cube partition of $\R^{d-1}$ (with coordinates indexed by $[d]\setminus\set{i_0}$). Thus, there is some layer coordinate $i_1\in[d]\setminus\set{i_0}$ for $\P'$ and some $\alpha\in\R$ such that
\[
\set{\centr_{i_1}(Y)\colon Y\in\P'} = \alpha+\Z.
\]
Now note the following:
\begin{align*}
\set{\centr_{i_1}(X)\colon X\in\P} &= \set{\centr_{i_1}(\tau_{i_0}(X))\colon X\in\P} \tag{center in $i_0$ unaffected by removal of $i_1$th coord since $i_0\not=i_1$} \\
    %
    &= \set{\centr_{i_1}(Y)\colon Y\in\P'} \\
    %
    &= \alpha+\Z
\end{align*}
which shows that $\P$ is a layer unit cube partition with layer coordinate $i_1$ (i.e. the layer coordinate $i_1$ of $\P'$ is also a layer coordinate of $\P$ because $\P$ looks like $\P'$ except that cubes have become stacks of cubes in the irrelevant coordinate $i_0$).

Now we must further show that $\P$ is a {\em recursively} layered unit cube partition with layer coordinate $i_1$. That is, we must show that for any $\beta\in\R$ that $P_{\hp{i_1}{\beta}}$ is a recursive layer unit cube partition. By \Autoref{recursive-tower-to-hyperplane}, because $\P$ is a recursive tower unit cube partition of $\R^d$, $P_{\hp{i_1}{\beta}}$ is a recursive tower unit cube partition of $\R^{d-1}$, so by inductive hypothesis, $P_{\hp{i_1}{\beta}}$ is a recursive layer unit cube partition of $\R^{d-1}$.
% That is, we must show for any $n\in\Z$ that the set
% \[
% \P''\defeq\set{\tau_{i_1}(X)\colon X\in\P\text{ and }\center_{i_1}(X)=\alpha+n}
% \]
% is a recursive layer partition of $\R^{d-1}$.

% We will justify that
% \[
% \P''=\P_{\hp{i_1}{\alpha}}.
% \]
\end{proof}

\begin{proposition}[Lattice $\Longrightarrow$ Recursive Tower]\label{lattice-is-recursive-tower}
Let $d\in\N$ and $\P$ a lattice unit cube partition of $\R^d$. Then $\P$ is also a recursive tower unit cube partition of $\R^d$.
\end{proposition}
\begin{proof}

\end{proof}

\begin{example}[Tower $\not\Longrightarrow$ Layer]\label{tower-not-layer}

\end{example}


\todo[inline]{Explore this to try to prove this. It would be good to know so that some of our bounds also apply to the Hoza-Klivans partitions}
\begin{conjecture}[Hoza-Klivans Partition]
For each $d\in\N$, the scaled Hoza-Klivans partition of $\R^d$ is a single set unit lattice partition.
\end{conjecture}

%
% THIS CONJECTURE HAS BEEN MOVED TO LATER
%
% \begin{conjecture}[Bubble Measure Increase]
% Let $d\in\N$, and $S\subseteq\R^d$ be any Lebesgue measurable set with $m(S)=1$. Then for any $\epsilon\in[0,\infty)$, $m(\bubble_{\epsilon}(S))\geq(1+2\epsilon)^d$ (where $\bubble_{\epsilon}$ is with respect to $\ell_{\infty}$).
% \end{conjecture}

\begin{conjecture}[Exponential $k$ for Lattice Partitions]
Let $d,k\in\N$ and $\epsilon\in[0,\frac12]$. If $\P$ is a single set lattice unit partition of $\R^d$ which is $(k,\epsilon)$-secluded, then $k\geq(1+2\epsilon)^d$.
\end{conjecture}
If the Bubble Measure Increase conjecture is true, then this conjecture is true using Blichfeldt's theorem and my Antisymmetry Containment Lemma



\subsection{Single Set Partitions}

While we have had success in proving results for a variety of types of unit cube partitions, we have (unsurprisingly) found it harder to prove results for generic partitions (even if we consider a uniform bound on the measure and/or diameter of all members or consider some type of local finiteness as in our previous paper). However, we can generalize our results by considering that many of the partitions used in practice in theoretical computer science have members that in a precise sense are positioned on a lattice. For example, all partitions of [[the foams paper]] are positioned on the standard integer lattice $\Z^d$, and the partition of Hoza and Klivans also has all members positioned on the integer lattice $\Z^d$. Thus, we could consider partitions of this form. However, we are able to generalize even further than this to ignore the fact that there is an underlying algebraic lattice structure to the positions of the members and focus only on the fact that each member of these partitions is identical up to a translation. We formally define the class of such partitions below.

\begin{definition}[Single Set Partition]
Let $d\in\N$. A {\em single set partition} $\P$ of $\R^d$ is a partition of $\R^d$ such that there exists a set $S\subseteq\R^d$, and for every $X\in\P$, there exists some $\vec{x}\in\R^d$ (not necessarily unique) such that $X=\vec{x}+S$.
\end{definition}

\begin{remark}\label{non-unique-rep}
For many natural sets, the $\vec{x}$ in the definition above will be unique, but for example, $\R^d$ can be partitioned into translates of $\Z^d$, so for any $X$ in such a partition and any$\vec{n}\in\Z^d$, $\vec{x}+X = \vec{x}+\vec{n}+X$.
\end{remark}

For a single set partition $\P$, it will be convenient to have a function which returns a single representative point of each member of $\P$, and furthermore, since every member of the partition is a translate of a common set, we want this function to return the ``same'' point for each member.

\begin{definition}[Representative Function]\label{defn-rep-fun}
Let $d\in\N$ and $\P$ be a single set partition of $\R^d$ using the set $S\subseteq\R^d$. A {\em representative function} is a function $\rep:\P\to\R^d$ with the property that for any $X,Y\in\P$, we have $X-\rep(X)=Y-\rep(Y)$. 
\end{definition}

Intuitively, the definition above requires that translating $X$ so that its representative is at the origin and translating $Y$ so that its representative is at the origin result in the same set. Even more informally, $\rep(X)$ is the same point relative to $X$ as $\rep(Y)$ is to $Y$. An alternative way we could have defined this is to fix some $\vec{s}\in S$ and note that for each $X\in\P$, $X=S+\vec{x}$ for some $\vec{x}\in\R^d$, and we could define $\rep(X)$ to be $\vec{x}$. The problem with this approach is that one may have to choose which $\vec{x}$ this is due to \Autoref{non-unique-rep}.

\begin{remark}
In the above definition, we do not require that $\rep(X)\in X$, as we won't need that property for any of our results, but from the perspective of partitions as rounding schemes, it would be natural (though, again, not necessary) that $\rep(X)\in X$ so that all points in the member $X$ are rounded to the value $\rep(X)$.
\end{remark}

As with unit cube partitions, we will be interested in considering for each $\vec{p}\in\R^d$, the $\epsilon$ neighborhood $\neigh{\epsilon}{\vec{p}}=\set{X\in\P\colon X\cap\ballc{\epsilon}{\vec{p}}\not=\empty}$. The following important result will allow us to examine this neighborhood without considering the $\epsilon$ ball directly. Instead, we can consider only the representative of each member along with a certain large measurable set $B$; we can equivalently characterize the collection $\neigh{\epsilon}{\vec{p}}$ as consisting of exactly the members of $\P$ whose representative is contained in the set $B$. This perspective allows us to discretize the problem of understanding $\neigh{\epsilon}{\vec{p}}$.

% \begin{lemma}[Antisymmetry Containment]
% Let $d\in\N$ and $S\subseteq\R^d$. Let $\mathcal{A}=\set{\vec{\alpha}+S\colon\vec{\alpha}\in\R^d}$ be all shifts of the set $S$. Let $\rep:\mathcal{A}\to\R^d$ be any function such that for all $\vec{\alpha}\in\R^d$, it holds that $\rep(\vec{\alpha}+S)=\vec{\alpha}+\rep(S)$. Let $\P$ be a partition of $\R^d$ such that $\P\subseteq\mathcal{A}$. Let $B=\bubble_{\epsilon}(-S+\rep(S))$. Then for all $\epsilon\in[0,\infty)$ and all $\vec{p}\in\R^d$ the following holds:
% \[
%     \neigh{\epsilon}{\vec{p}} = \set{X\in\P\colon \rep(X)\in \vec{p}+B}
% \]
% \end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This result has been generalized and moved to general_bounds.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \todo[inline]{Formalize the hyptheses of this claim}
% \begin{claim}\label{antisymmetry-containment-pre-claim}
% \[
% \ballc{\epsilon}{\vec{p}}\cap X\not=\emptyset \iff \vec{p}\in\bubble_{\epsilon}(X)
% \]
% \end{claim}
% \begin{proof}
% ($\Longrightarrow$) If $\ballc{\epsilon}{\vec{p}}\cap X\not=\emptyset$, then there exists $\vec{y}\in\ballc{\epsilon}{\vec{p}}\cap X$, and since $\vec{y}\in\ballc{\epsilon}{\vec{p}}$ we have $d_{max}(\vec{y},\vec{p})\leq\epsilon$ so $\vec{p}\in\ballc{\epsilon}{\vec{y}}\subseteq\bigcup_{\vec{x}\in X}\ballc{\epsilon}{\vec{x}}=\bubble_{\epsilon}(X)$

% ($\Longleftarrow$) If $\vec{p}\in\bubble_{\epsilon}(X)$, then there exists $\vec{y}\in X$ such that $\vec{p}\in\ballc{\epsilon}{\vec{y}}$, so $d_{max}(\vec{p},\vec{y})\leq\epsilon$ so $\vec{y}\in\ballc{\epsilon}{\vec{p}}$, so $\vec{y}\in\ballc{\epsilon}{\vec{p}}\cap X$ implying that $\ballc{\epsilon}{\vec{p}}\cap X\not\emptyset$.
% \end{proof}
% \begin{fact}\label{antisymmetry-containment-pre-claim-minkowski-sum}
% Let $d\in\N_1$ and $X\subseteq\R^d$ and $\vec{p}\in\R^d$. Then
% \[
% \ballc{\epsilon}{\vec{p}}\cap X\not=\emptyset \iff \vec{p}\in X+\ballc{\epsilon}{\vec{0}}.
% \]
% \end{fact}
% \begin{proof}
% ($\Longrightarrow$) If $\ballc{\epsilon}{\vec{p}}\cap X\not=\emptyset$, then there exists $\vec{y}\in\ballc{\epsilon}{\vec{p}}\cap X$, and since $\vec{y}\in\ballc{\epsilon}{\vec{p}}$ we have $d_{max}(\vec{y},\vec{p})\leq\epsilon$ so $\vec{p}\in\ballc{\epsilon}{\vec{y}}=\vec{y}+\ballc{\epsilon}{\vec{0}}$, and since $\vec{y}\in X$, $\vec{y}+\ballc{\epsilon}{\vec{0}}\subseteq X+\ballc{\epsilon}{\vec{0}}$ showing that $\vec{p}\in X+\ballc{\epsilon}{\vec{0}}$.

% ($\Longleftarrow$) If $\vec{p}\in X+\ballc{\epsilon}{\vec{0}}$ then there exists $\vec{x}\in X$ and $\vec{b}\in\ballc{\epsilon}{\vec{0}}$ such that $\vec{p}=\vec{x}+\vec{b}$. Thus $\vec{x}=\vec{p}-\vec{b}\in\ballc{\epsilon}{\vec{p}}$ showing that $\vec{x}$ belongs to both $X$ and $\ballc{\epsilon}{\vec{p}}$ so that their intersection is non-empty.
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This result has been moved to general_bounds.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{fact}\label{minkowski-bubble-union}
% $X+\ballc{\epsilon}{\vec{0}} = \bigcup_{\vec{x}\in X}\ballc{\epsilon}{\vec{x}}$ and $X+\ballo{\epsilon}{\vec{0}} = \bigcup_{\vec{x}\in X}\ballo{\epsilon}{\vec{x}}$.
% \end{fact}
% \begin{proof}
% We prove only the closed version as the proof of the open version is identical.

% ($\subseteq$) A generic element of $X+\ballc{\epsilon}{\vec{0}}$ is $\vec{x}+\vec{b}$ for some $\vec{x}\in X$ and $\vec{b}\in \ballc{\epsilon}{\vec{0}}$ which means $\vec{x}+\vec{b}\in\vec{x}+\ballc{\epsilon}{\vec{0}}=\ballc{\epsilon}{\vec{x}}\subseteq \bigcup_{\vec{x}\in X}\ballc{\epsilon}{\vec{x}}$.

% ($\supseteq$) Given $\vec{y}\in \bigcup_{\vec{x}\in X}\ballc{\epsilon}{\vec{x}}$ there is some particular $\vec{x}\in X$ such that $y\in\ballc{\epsilon}{\vec{x}}=\vec{x}+\ballc{\epsilon}{\vec{0}}$ which means $\vec{y}=\vec{x}+\vec{b}$ for some $\vec{b}\in \ballc{\epsilon}{\vec{0}}$, and since $\vec{x}\in X$, we have $\vec{y}\in X+\ballc{\epsilon}{\vec{0}}$.
% \end{proof}


\begin{lemma}[Antisymmetry Containment]
Let $d\in\N$ and $\P$ a single set partition of $\R^d$ and $\rep:\P\to\R^d$ a representative function, and $S$ an arbitrary member of $\P$. Define $B=-\bubble_{\epsilon}(S-\rep(S))$ (noting that by the definition of representative functions, $B$ is invariant under the choice of $S$). Then for all $\epsilon\in[0,\infty)$ and all $\vec{p}\in\R^d$ the following holds:
\[
    \neigh{\epsilon}{\vec{p}} = \set{X\in\P\colon \rep(X)\in \vec{p}+B}
\]
\end{lemma}
\begin{proof}
We have the following set equalitites:
\begin{align*}
    \neigh{\epsilon}{\vec{p}} 
    &= \set{X\in\P\colon \ballc{\epsilon}{\vec{p}}\not=\emptyset} \tag{By definition} \\
    &= \set{X\in\P\colon \vec{p}\in\bubble_{\epsilon}(X)} \tag{By \Autoref{antisymmetry-containment-pre-claim}} \\
    &= \set{X\in\P\colon -\left(\rep(X)-\vec{p}\right)+\rep(X) \in\bubble_{\epsilon}(X)} \tag{Add and subtract $\rep(X)$ to $\vec{p}$} \\ 
    &= \set{X\in\P\colon -\left(\rep(X)-\vec{p}\right) \in\bubble_{\epsilon}(X)-\rep(X)} \tag{Apply shift of $-\rep(X)$ to point and set} \\
    &= \set{X\in\P\colon \rep(X)-\vec{p} \in -(\bubble_{\epsilon}(X)-\rep(X))} \tag{Negate point and set} \\
    &= \set{X\in\P\colon \rep(X) \in -(\bubble_{\epsilon}(X)-\rep(X))+\vec{p}} \tag{Apply shift of $\vec{p}$ to point and set} \\
    &= \set{X\in\P\colon \rep(X) \in -(\bubble_{\epsilon}(X-\rep(X)))+\vec{p}} \tag{A basic algebraic equality for $\bubble$} \\
    &= \set{X\in\P\colon \rep(X) \in -(\bubble_{\epsilon}(S-\rep(S)))+\vec{p}} \tag{Def'n of $\rep$ (\Autoref{defn-rep-fun})} \\
    &= \set{X\in\P\colon \rep(X)\in \vec{p}+B} \tag{Def'n of $B$}
\end{align*}
\end{proof}


The prior result made use of the $\epsilon$ bubble around a set, and as we will later make use of that result, we wish to know something about the measure of the $\epsilon$ bubble around a set $S$ (assuming $S$ is measurable) relative to the measure of $S$. We do so in the following result, and then we follow this up with a conjecture of a stronger result.

\begin{lemma}[Bubble Measure Lemma]
Let $d\in\N$ and $S\subseteq\R^d$ with $D=\diam(S)<\infty$ (the diameter taken with respect to the $\ell_\infty$ norm/$d_{max}$ metric). Then for any $\epsilon\in[0,\infty)$,
\[
    m\left(\bubble_{\epsilon}(S)\right) \geq \left(1+\frac{2\epsilon}{D}\right)^d\cdot m(S).
\]
\end{lemma}
\begin{proof}
By \Autoref{diameter-ball}, since the diameter of $S$ is $D$ with respect to $\ell_\infty$, there exists $\vec{\alpha}\in\R^d$ such that $S\subseteq\ballc{D/2}{\vec{\alpha}}$, so by translation by $-\vec{\alpha}$ we have $S-\vec{\alpha}\subseteq\ballc{D/2}{\vec{0}}$.

We now show that $\left(1+\frac{2\epsilon}{D}\right)\cdot\left(S-\vec{\alpha}\right)\subseteq\bubble_{\epsilon}(S-\vec{\alpha})$. Consider an arbitrary $\vec{y}\in\left(1+\frac{2\epsilon}{D}\right)\cdot\left(S-\vec{\alpha}\right)$. Then there is some $\vec{x}\in S-\vec{\alpha}\subseteq\ballc{D/2}{\vec{0}}$ such that $\vec{y}=\left(1+\frac{2\epsilon}{D}\right)\cdot\vec{x}$. Since $\vec{x}\in\ballc{D/2}{\vec{0}}$, we have $\norm{\vec{x}}_\infty\leq\frac{D}{2}$ which means that for all $i\in[d]$, $x_i\in[-\frac{D}{2},\frac{D}{2}]$. Thus, for each $i\in[d]$,
\[
y_i = \left(1+\frac{2\epsilon}{D}\right)\cdot\vec{x} = x_i + \frac{2\epsilon}{D}\cdot\vec{x} \in x_i + \frac{2\epsilon}{D}[-\frac{D}{2},\frac{D}{2}] = x_i+[-\epsilon,\epsilon].
\]
This shows that $\vec{y}\in\ballc{\epsilon}{\vec{x}}\subseteq\bigcup_{\vec{z}\in S-\vec{\alpha}}\ballc{\epsilon}{\vec{z}}=\bubble_{\epsilon}(S-\vec{\alpha})$.
Since $\vec{y}$ was arbitrary, this shows that $\left(1+\frac{2\epsilon}{D}\right)\cdot\left(S-\vec{\alpha}\right)\subseteq\bubble_{\epsilon}(S-\vec{\alpha})$.

With this, we have the following inequalities:
\begin{align*}
    m(\bubble_{\epsilon}(S)) &= m(\bubble_{\epsilon}(S)-\vec{\alpha}) \tag{Lebesgue measure is translation invariant} \\
     &= m(\bubble_{\epsilon}(S-\vec{\alpha})) \tag{A basic algebraic set equality for $\bubble$} \\
     &\geq m\left(\left(1+\frac{2\epsilon}{D}\right)\cdot\left(S-\vec{\alpha}\right)\right) \tag{Monotonicity of measures for subsets} \\
     &\geq m\left(\left(1+\frac{2\epsilon}{D}\right)\cdot S-\left(1+\frac{2\epsilon}{D}\right)\cdot\vec{\alpha}\right) \tag{Set equality} \\
     &= m\left(\left(1+\frac{2\epsilon}{D}\right)\cdot S\right) \tag{Lebesgue measure is translation invariant} \\
     &= \left(1+\frac{2\epsilon}{D}\right)^d\cdot m\left(S\right) \tag{Lebesgue measure of scaled set} \\
\end{align*}
This completes the proof.
\end{proof}


%
% THE CONJECTURE BELOW IS OBVIOUSLY FALSE BC IF THE DIAMETER IS MASSIVE, THEN THE EPSILON BUBBLE (FOR SMALL EPSILON) WILL DO VIRTUALLY NOTHING TO THE VOLUME. I REALLY MEANT FOR THE CONJECTURE TO BE TRUE FOR ___UNIT VOLUME___ SETS, AND FOR THESE IT MIGHT STILL BE TRUE
%
\begin{conjecture}[Bubble Measure Conjecture]
% Let $d\in\N$, and $S\subseteq\R^d$ be any Lebesgue measurable set with $m(S)=1$. Then for any $\epsilon\in[0,\infty)$, $m(\bubble_{\epsilon}(S))\geq(1+2\epsilon)^d$ (where $\bubble_{\epsilon}$ is with respect to $\ell_{\infty}$).
Let $d\in\N$ and $S\subseteq\R^d$ be measurable with $m(S)\leq1$ and have finite diameter $\diam(S)<\infty$ (the diameter taken with respect to the $\ell_\infty$ norm/$d_{max}$ metric). Then for any $\epsilon\in[0,\infty)$,
\[
    m\left(\bubble_{\epsilon}(S)\right) \geq \left(1+2\epsilon\right)^d\cdot m(S).
\]
\end{conjecture}

\begin{remark}
We do not claim the above conjecture for any metric/norm except for $\ell_\infty$. In particular the conjecture is false for the $\ell_2$ norm even in $\R^2$. \todo[inline]{Elaborate with circle example}

The purpose of the conjecture is to allow us to normalize a partition based on the measure instead of based on the diameter.
\end{remark}




\begin{theorem}[Generalized Blichfeldt's Theorem]\label{generalized-blichfeldt}
Let $d\in\N$ and $\P$ a single set partition of $\R^d$ and $\rep:\P\to\R^d$ a representative function, and $S$ an arbitrary member of $\P$ and $B\subseteq\R^d$ a measurable set. If $S$ is measurable with finite measure, then there exists $\vec{p}\in\R^d$ such that $\vec{p}+B$ contains at least $\ceil{\frac{m(B)}{m(S)}}$ representative points. That is,
% \[
%     \abs{\set{\rep(X):X\in\P} \cap (\vec{p}+B)} \geq \ceil{\frac{m(B)}{m(S)}}.
% \]
\[
    \abs{\set{\rep(X):X\in\P\text{ and }\rep(X)\in \vec{p}+B)}} \geq \ceil{\frac{m(B)}{m(S)}}.
\]
\end{theorem}
\begin{proof}

\end{proof}

\begin{theorem}[Single Set Partition Bound]\label{single-set-partition-bound}
Let $d\in\N$ and $\P$ a single set partition of $\R^d$ and $S$ an arbitrary member of $\P$. If $S$ is measurable and has finite measure and finite diameter $D=\diam(S)$ (with respect to $\ell_\infty$), then for any $\epsilon\in[0,\infty)$, there exists $\vec{p}\in\R^d$ such that 
\[
    \abs{\neigh{\epsilon}{\vec{p}}}\geq\ceil{(1+2\epsilon)^d}.
\]
\end{theorem}
\begin{proof}

\end{proof}

==> proofs_for_l_infty_norm_specifically.tex <==
\begin{lemma}\label{outer-measure-brunn-minkowsi-bound}
Let $d\in\N_1$, $Y\subseteq\R^d$, and $\epsilon\in(0,\infty)$. Then $Y+\ballo{\epsilon}{\vec{0}}$ is open (and thus Borel measurable), and $m(Y+\ballo{\epsilon}{\vec{0}})\geq \left([m_{out}(Y)]^\frac1d+2\epsilon\right)^d$.
\end{lemma}
\begin{proof}
By \Autoref{minkowski-bubble-union}, $Y+\ballo{\epsilon}{\vec{0}}=\bigcup_{\vec{y}\in Y}\ballo{\epsilon}{\vec{y}}$  which is a union of open sets, so is itself open and thus Borel measurable.

Now, for any $\epsilon'\in(0,\epsilon)$, observe that by \Autoref{sum-of-balls}, $\ballo{\epsilon}{\vec{0}}=\ballo{\epsilon-\epsilon'}{\vec{0}}+\ballo{\epsilon'}{\vec{0}}$ and thus, this sum is measurable because it is an open ball. 

Now, using the above equality and the associativity of the Minkowski sum, we have 
\[
Y+\ballo{\epsilon}{\vec{0}} = Y + \left[\ballo{\epsilon-\epsilon'}{\vec{0}}+\ballo{\epsilon'}{\vec{0}}\right] = \left[Y + \ballo{\epsilon-\epsilon'}{\vec{0}}\right] +\ballo{\epsilon'}{\vec{0}}.
\]
Thus, we have the following inequalities:
\begin{align*}
    m\left(Y+\ballo{\epsilon}{\vec{0}}\right) &= m\left(\left[Y + \ballo{\epsilon-\epsilon'}{\vec{0}}\right] +\ballo{\epsilon'}{\vec{0}}\right) \tag{Above} \\
    %
    %
    &\geq 
    \left( 
        \left[m\left(Y + \ballo{\epsilon-\epsilon'}{\vec{0}}\right)\right]^{\frac1d}
        +
        \left[
            m\left(\ballo{\epsilon'}{\vec{0}}\right)
        \right]^{\frac1d}
    \right)^d
    \tag{Generalized Brunn-Minkowski (\Autoref{generalized-brunn-minkowski-inequality})} \\
    %
    %
    &= 
    \left( 
        \left[m\left(Y + \ballo{\epsilon-\epsilon'}{\vec{0}}\right)\right]^{\frac1d}
        +
        \left[
            (2\epsilon')^d
        \right]^{\frac1d}
    \right)^d
    \tag{$\ballo{\epsilon'}{\vec{0}}=[-\epsilon',\epsilon']^d$} \\
    %
    %
    &= 
    \left( 
        \left[m\left(Y + \ballo{\epsilon-\epsilon'}{\vec{0}}\right)\right]^{\frac1d}
        +
        2\epsilon'
    \right)^d
    \tag{Simplify} \\
    %
    %
    &\geq
    \left( 
        \left[m_{out}\left(Y\right)\right]^{\frac1d}
        +
        2\epsilon'
    \right)^d
    \tag{$m_{out}$ is infimum of measures of measurable supersets}
\end{align*}
Since the above holds for all any $\epsilon'\in(0,\epsilon)$, by continuity, the inequality also holds for $\epsilon'=\epsilon$ (see footnote\footnote{To see this, suppose for contradiction that $m\left(Y+\ballo{\epsilon}{\vec{0}}\right)<\left(\left[m_{out}\left(Y\right)\right]^{\frac1d} + 2\epsilon\right)^d$. Since $\left(\left[m_{out}\left(Y\right)\right]^{\frac1d} + 2\epsilon'\right)^d$ is a continuous function of $\epsilon'$ for fixed $Y$ and $d$, we can find $\epsilon'\in(0,\epsilon)$ such that $m\left(Y+\ballo{\epsilon}{\vec{0}}\right) < \left(\left[m_{out}\left(Y\right)\right]^{\frac1d} + 2\epsilon'\right)^d < \left(\left[m_{out}\left(Y\right)\right]^{\frac1d} + 2\epsilon\right)^d$ which contradicts the inequalities in the proof for such $\epsilon'$.}) giving the desired conclusion.
\end{proof}




\begin{theorem}[$\epsilon$-Neighborhoods for Measure Bounded Partitions]\label{epsilon-measure-bounded}
Let $d\in\N_1$, $M\in[0,\infty)$, and $\P$ a partition of $\R^d$ such that every member has outer Lebesgue measure at most $M$. Let $\epsilon\in[0,\infty)$. Then there exists $\vec{p}\in\R^d$ such that $\abs{\neigh{\epsilon}{\vec{p}}}\geq\ceil*{\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d}$.
\end{theorem}
\begin{proof}
\renewcommand{\A}{\mathcal{A}}
\newcommand{\F}{\mathcal{F}}
Consider the following for each $n\in\N_1$. Let $S_n=[-n,n]^d$ and $S_n'=[-n-\epsilon,n+\epsilon]^d$ and $\S$ be the partition of $S_n$ induced by $\P$ (i.e. $\S=\set{X\cap S_n\colon X\in\P\text{ and }X\cap S_n\not=\emptyset}$). For each $Y\in\S_n$, let $C_{Y}=Y+\ballo{\epsilon}{\vec{0}}$. By \Autoref{outer-measure-brunn-minkowsi-bound}, $C_Y$ is measurable, and $m(C_Y)\geq \left(\left[m_{out}\left(Y\right)\right]^{\frac1d} + 2\epsilon\right)^d$. Also observe that $C_Y\subseteq S_n'$. Now consider the following inequalities:
\begin{align*}
    m(C_Y) &\geq \left(\left[m_{out}\left(Y\right)\right]^{\frac1d} + 2\epsilon\right)^d \tag{Above} \\  %
    %
    &= \left(M^{1/d}\left[\frac{\left[m_{out}\left(Y\right)\right]^{\frac1d}}{M^{1/d}} + \frac{2\epsilon}{M^{1/d}}\right]\right)^d \tag{Algebra} \\
    %
    %
    &= M\left(\left[\frac{m_{out}\left(Y\right)}{M}\right]^{\frac1d} + \frac{2\epsilon}{M^{1/d}}\right)^d \tag{Algebra} \\
    %
    %
    &= M\cdot \frac{m_{out}\left(Y\right)}{M} \cdot \left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \tag{\Autoref{brunn-minkowski-bound-lemma} since $\frac{m_{out}\left(Y\right)}{M}\in[0,1]$} \\
    %
    %
    &= m_{out}\left(Y\right)\cdot\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \tag{Simplify} \\
\end{align*}
The above shows that for each $Y\in\S_n$, the set $Y+\ballo{\epsilon}{\vec{0}}$ has substantially more (a factor of $\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d$) content than $Y$ does. We will extend this to unsurprisingly show that this implies that $\set{Y+\ballo{\epsilon}{\vec{0}}}_{Y\in\S_n}$ also has this same factor more content than $\S_n$ does, observing that $\S_n$ has total content of about $m(S_n)$ since $\S_n$ is a partition of $S_n$ (any discrepency is due to non-measurable members in $\S_n$)

Formally, we claim that there exists a finite subfamily $\F_n\subseteq\S_n$ such that
\[
\sum_{Y\in\F_n}m\left(Y+\ballo{\epsilon}{\vec{0}}\right) \geq \left(1+\frac{2\epsilon}{M^{1/d}}\right)^d\cdot m(S_n).
\]
To see this, first consider the case that $\S_n$ has infinite cardinality. Let $\F_n\subset\S_n$ be any subfamily of $\frac{\ceil{\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d\cdot m(S_n)}}{(2\epsilon)^d}$-many sets noting that
\begin{align*}
    \sum_{Y\in\F_n}m\left(Y+\ballo{\epsilon}{\vec{0}}\right) &\geq \sum_{Y\in\F_n}m\left(\ballo{\epsilon}{\vec{0}}\right) \tag{$Y+\ballo{\epsilon}{\vec{0}}$ is a superset of a translation of $\ballo{\epsilon}{\vec{0}}$ since $Y\not=\emptyset$} \\
    &= \sum_{Y\in\F_n}(2\epsilon)^d \tag{$\ballo{\epsilon}{\vec{0}}=[-\epsilon,\epsilon]^d$} \\
    &= \frac{\ceil{\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d\cdot m(S_n)}}{(2\epsilon)^d} \cdot (2\epsilon)^d \tag{Cardinality of $\F_n$}\\
    &= \ceil{\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d\cdot m(S_n)} \tag{Simplify}.
\end{align*}
Now consider the other case where $\S_n$ has finite cardinality\footnote{In fact this case also works if $\S_n$ is countable even though we have already dealt with that case.}. Take $\F_n=\S_n$ so that
\begin{align*}
    \sum_{Y\in\F_n}m\left(Y+\ballo{\epsilon}{\vec{0}}\right) &=     \sum_{Y\in\S_n}m\left(Y+\ballo{\epsilon}{\vec{0}}\right) \tag{$\F_n=\S_n$} \\
    &\geq \sum_{Y\in\S_n}m_{out}\left(Y\right)\cdot\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \tag{Above}\\
    &= \left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot \sum_{Y\in\S_n}m_{out}\left(Y\right) \tag{Linearity of summation} \\
    &\geq \left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot m_{out}\left(\bigcup_{Y\in\S_n}Y\right) \tag{Countable subaddativity of outer measures} \\
    &= \left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot m\left(S_n\right) \tag{$S_n=\bigsqcup_{Y\in\F_n}Y$ is measurable}
\end{align*}

% Now, by \Autoref{lower-bound-cover-number} (see footnote for details\footnote{}), there is a point 

So letting $\F_n\subseteq\S_n$ be such a finite family, let $\A_n=\set{Y+\ballo{\epsilon}{\vec{0}}}_{Y\in\F_n}$ be a family indexed\footnote{We require this to be an indexed family rather than just a set, because it is possible that there are distinct $Y,Y'\in\S_n$ such that $Y+\ballo{\epsilon}{\vec{0}}=Y'+\ballo{\epsilon}{\vec{0}}$.} by $\F_n$.

Again, we note that for each $A\in\A_n$, $A\subseteq S_n'=[-n-\epsilon,n+\epsilon]^d$. Thus, by \Autoref{lower-bound-cover-number}\footnote{We are taking $X$ in \Autoref{lower-bound-cover-number} to be $S_n'=[-n-\epsilon,n+\epsilon]^d$ in this proof, and taking $\mu$ to be $m$ and taking $\A$ to be $\A_n$. We have that $\sum_{A\in\A_n}m(A)<\infty$ because $\abs{\A_n}=\abs{\F_n}$ is finite, and each $A\in\A_n$ is a subset of $S_n'$, so has finite measure.}, there is a point $\vec{p}^{(n)}\in S_n'$ which belongs to at least the following number of sets in $\A$:
\begin{align*}
\frac{\sum_{Y\in\F_n}m\left(Y+\ballo{\epsilon}{\vec{0}}\right)}{m(S_n')} &\geq \frac{\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot m\left(S_n\right)}{m(S_n')} \\
&= \left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot \frac{(2n)^d}{(2(n+\epsilon))^d} \\
&= \left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot \left(\frac{n}{n+\epsilon}\right)^d.
\end{align*}

For each $Y\in\F_n\subseteq\S_n$ for which $\vec{p}^{(n)}\in Y+\ballo{\epsilon}{\vec{0}}$, we trivially have $\vec{p}^{(n)}\in Y+\ballc{\epsilon}{\vec{0}}$, so by \Autoref{antisymmetry-containment-pre-claim-minkowski-sum}, we have $Y\cap\ballc{\epsilon}{\vec{0}}\not=\emptyset$. For each such $Y$, there is a distinct $X_Y\in\P$ such that $Y\subseteq X_Y$ and thus $X_Y\cap\ballc{\epsilon}{\vec{0}}\not=\emptyset$ showing that $X_Y\in\neigho{\epsilon}{\vec{p}^{(n)}}$. Since there are at least $\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot \left(\frac{n}{n+\epsilon}\right)^d$-many such $Y$, we have
\[
\abs{\neigho{\epsilon}{\vec{p}^{(n)}}} \geq \left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot \left(\frac{n}{n+\epsilon}\right)^d.
\]

For the last step of the proof, we perform a limiting process on $n$. By \Autoref{smaller-ceiling}, let $\gamma\in\R$ such that $\gamma<\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d$ and $\ceil{\gamma}=\ceil{\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d}$. Then, because 
\[
\lim_{n\to\infty}\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot \left(\frac{n}{n+\epsilon}\right)^d = \left(1+\frac{2\epsilon}{M^{1/d}}\right)^d > \gamma,
\]
we can take $N\in\N_1$ sufficiently large so that
\[
\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d \cdot \left(\frac{N}{N+\epsilon}\right)^d > \gamma.
\]
Then $\abs{\neigh{\epsilon}{\vec{p}^{(N)}}} \geq \gamma$, and since the cardinality is either infinite or an integer, we can take the ceiling on the right hand side, so by the choice of $\gamma$, we have
\[
    \abs{\neigh{\epsilon}{\vec{p}^{(N)}}} \geq \ceil{\gamma} = \ceil{\left(1+\frac{2\epsilon}{M^{1/d}}\right)^d}
\]
which completes the proof.
\end{proof}

==> sperner_kkm_lebesgue_figure.tex <==
% This looks more complicated than normal in order to display the figure numbers with priority for moving down the columns instead of across the rows. 
% https://tex.stackexchange.com/questions/235690/i-want-to-change-the-order-of-numbering-for-captions-in-subfigure
% https://tex.stackexchange.com/questions/31823/how-to-reference-subfigure-in-caption
\begin{figure}[p]
\sbox1{%
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/sperner_kkm_lebesgue/1_non_spanning_coloring.png}
        \subcaption{Initial coloring $\chi$}
        \label{subfig:1_non_spanning_coloring}
    \end{subfigure}
}
\sbox2{%
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/sperner_kkm_lebesgue/2_extended_coloring.png}
        \subcaption{Extended coloring $\gamma$}
        \label{subfig:2_extended_coloring}
    \end{subfigure}
}
\sbox3{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/sperner_kkm_lebesgue/3_red.png}
        \subcaption{Red points ($Y_{\text{red}}$)}
        \label{subfig:3_red}
    \end{subfigure}
}
\sbox4{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/sperner_kkm_lebesgue/4_red.png}
        \subcaption{Ball added ($Y_{\text{red}}+B_{\vec{v}}$)}
        \label{subfig:4_red}
    \end{subfigure}
}
\sbox5{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/sperner_kkm_lebesgue/5_purple.png}
        \subcaption{Purple points ($Y_{\text{purple}}$)}
        \label{subfig:5_purple}
    \end{subfigure}
}
\sbox6{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/sperner_kkm_lebesgue/6_purple.png}
        \subcaption{Ball added ($Y_{\text{purple}}+B_{\vec{v}}$)}
        \label{subfig:6_purple}
    \end{subfigure}
}
\sbox7{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/sperner_kkm_lebesgue/7_gray.png}
        \subcaption{Gray points ($Y_{\text{gray}}$)}
        \label{subfig:7_gray}
    \end{subfigure}
}
\sbox8{
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=\textwidth]{images/sperner_kkm_lebesgue/8_gray.png}
        \subcaption{Ball added ($Y_{\text{gray}}+B_{\vec{v}}$)}
        \label{subfig:8_gray}
    \end{subfigure}
}
% \sbox9{%
%     \begin{subfigure}{.3\textwidth}
%         \includegraphics[width=\textwidth]{images/blank_square.png}
%     \end{subfigure}
% }
\sbox0{%
    \begin{subfigure}{.15\textwidth}
        \includegraphics[width=\textwidth]{images/sperner_kkm_lebesgue/blank_square.png}
    \end{subfigure}
}

\centering
\usebox0 \hfill \usebox1 \hfill \usebox2 \hfill \usebox0
\usebox3 \hfill \usebox5 \hfill \usebox7
\usebox4 \hfill \usebox6 \hfill \usebox8


\caption{
(\subref{subfig:1_non_spanning_coloring}) shows a (finite) coloring $\chi$ of the unit cube $[-\frac12,\frac12]^2$ such that no color includes points on opposite edges.
(\subref{subfig:2_extended_coloring}) shows the natural extension $\gamma$ of that coloring to $[-\frac12-\epsilon,\frac12+\epsilon]^2$. The extension is obtained by mapping each point $\vec{y}$ to the point $\vec{x}$ for which each coordinate value $y_i$ is restricted to be within $[-\frac12,\frac12]$, and then $\vec{y}$ is given whatever color $\vec{x}$ had.
% %
% Because no color included points on opposite edges in the initial coloring, in the extended coloring, each color is bounded $\epsilon$ away from one of the two directions in each coordinate. This means there is some quadrant of the $\ell_\infty$ $\epsilon$-ball that can be Miknowski summed with the color and the set remains a subset of the enlarged cube $[-\frac12-\epsilon,\frac12+\epsilon]^2$ as shown in the remaining subfigures.
% %
% \subref{subfig:3_red} shows the set of red points. Because it contains the upper left corner, the only quadrant of the ball that can be added to remain inside the extended cube is the bottom right quadrant. \subref{subfig:4_red} shows the resulting Minkowski sum which has substantially more area---by a factor of at least $(1+\frac{\epsilon}{1+\epsilon})^2$.
% %
% \subref{subfig:5_purple} and \subref{subfig:6_purple} are similar for purple.
% %
% For the gray points shown in \subref{subfig:7_gray} and \subref{subfig:8_gray}, there are actually two possible choices of the quadrant of the ball to use: the upper left quadrant or the upper right quadrant. The upper left is shown.
(\subref{subfig:3_red}), (\subref{subfig:5_purple}), and (\subref{subfig:7_gray}) show three of the five colors and demonstrate that there is at least one quadrant of the $\epsilon$-ball that can be Minkowski summed with the color so that the sum remains a subset of the extended cube. For red it is the lower right quadrant, for purple it is the upper right, and for gray it could be the upper left (shown) or the upper right. (\subref{subfig:4_red}), (\subref{subfig:6_purple}), and (\subref{subfig:8_gray}) show the resulting Minkowski sum for each color. Utilizing the Brunn-Minkowski inequality, this set will have substantially greater area---by a factor of at least $(1+\frac{\epsilon}{1+\epsilon})^2$.
}

\label{fig:sperner-kkm-coloring}

\end{figure}
